Hardware/Algorithm Co-design for Real-Time I/O Control with Improved Timing Accuracy and Robustness

In safety-critical systems, timing accuracy is the key to achieving precise I/O control. To meet such strict timing requirements, dedicated hardware assistance has recently been investigated and developed. However, these solutions are often fragile, due to unforeseen timing defects. In this paper, we propose a robust and timing-accurate I/O co-processor, which manages I/O tasks using Execution Time Servers (ETSs) and a two-level scheduler. The ETSs limit the impact of timing defects between tasks, and the scheduler prioritises ETSs based on their importance, offering a robust and configurable scheduling infrastructure. Based on the hardware design, we present an ETS-based timing-accurate I/O schedule, with the ETS parameters configured to further enhance robustness against timing defects. Experiments show the proposed I/O control method outperforms the state-of-the-art method in terms of timing accuracy and robustness without introducing significant overhead.

==> Discussions.tex <==
\section*{Discussions}

\noindent Background and Objectives:
\begin{itemize}
    \item In reality, we often cannot guarantee the WCET of a task always hold. That is, a task does occasionally exceed its WCET in real execution~\cite{hansen2009statistical, altmeyer2015wcet}. In a mixed-criticality system, when a task exceeds its WCET, the low criticality tasks are suspended to guarantee the timing of high-critical ones with a more pessimistic WCET estimation applied~\cite{burns2017survey}. 
    However, in a classic real-time system, tasks exceeding their WCETs can impose a significant impact on the system, and hence, jeopardising system schedulability~\cite{davis2007robust}. \textcolor{blue}{We might need to find some citations to justify the I/O jobs can exceed their WCETs. sensor examples might be better.}
    \item In our context, it undermines timing accuracy and schedulability as the I/O task exceeding its WCET can delay the pre-planned execution of the following tasks in the schedule produced by the state-of-the-art~\cite{zhao2020timing}. 
    \item This work propose a new I/O controller design and a robust I/O task scheduling mechanism (with analysis), which provides a safe margin for I/O tasks to exceed their WCETs while not affecting both timing accuracy and system schedulability.
\end{itemize}




\noindent Design Overvie:\\
\begin{itemize}
\item To present the high-level concept of our proposed design, we need a top-level diagram to illustrate our ideas. 
Therefore, I have drawn the diagram to illustrate the concepts.\\
There are a few topics that I wish to discuss regarding the concept diagram:\\
(i) How will we allocate the I/O jobs in the servers? Are they all dependent? \\
(ii) How will we show the servers can be dynamically generated or destroyed in the diagram? This is a key feature of the proposed design.\\
(iii) The diagram is a little bit simple at this monent. Is there anything else we can add?\\
\end{itemize}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{Overview.pdf}
    \caption{\name{}}
    \label{fig:concept1}
\end{figure}


\noindent Design Specs:\\
\begin{itemize}
\item The I/O controller is designed to support to execution mode: \\
(a). The configuration mode: where we can (i) configure the parameters of the servers, including priority, capacity, and period; (ii) pre-load the I/O jobs (name?).\\
(b). The operation mode: the I/O controllers operates the I/O jobs (name?), aligning with the configurations.

\item To support the two execution mode, we develop a communication protocol between the processor and the I/O controller. \\
(a) the new communication protocol defines a packet header for all I/O transactions.
(b) for I/O packets:

see below.

\begin{figure}[h]
    \centering
    \includegraphics[width=1\columnwidth]{Headers.pdf}
    \caption{Format of packet headers.}
    \label{fig:format}
\end{figure}

\item Now, let us introduce the top-level design of our I/O controller. \\
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{TopLevel_Controller.pdf}
    \caption{The top-level micro-architecture of the proposed I/O controller (black solid lines: operation paths; grey dash lines: configuration paths).}
    \label{fig:top}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{L-SE.pdf}
    \caption{Micro-architecture of the L-SE and its associated logic.}
    \label{fig:top}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{G-SE.pdf}
    \caption{Micro-architecture of the G-SE and its associated logic.}
    \label{fig:G-SE}
\end{figure}
\end{itemize}


\noindent Evaluation Plan:
\begin{itemize}
\item Performance (Timing accuracy and predictability), with/without tasks exceeding the WCETs (with a major focus on the ``with").
\item Hardware overhead -- compared to standardised I/O controllers, GPIOCP, RT-IOC.
\item Hardware scalability -- scaled with number of processors/I/Os.
\item Software overhead (can be done, do we need it?) \textcolor{blue}{There is no need to report software overhead as it is not the focus. We can simply provide time complexity of the allocation.}
\item A case study (if we have space) -- compared with software solutions x 2, GPIOCP, and RT-IOC. 
\end{itemize}


\noindent Major notes:
\begin{itemize}
\item We have a fixed number of servers during run-time.
\item SRAM to store offline and online packets. (minimum overhead).
\item \textcolor{red}{Need discussion on Sunday} Don't mind timing accuracy at the moment. Focusing on Robust I/O and schedulability first.
\item Naming of the packets, e.g., online/offline/configure packets.
\item Naming: I/O tasks, I/O jobs, metapackets, packets. \textcolor{blue}{(Important, we need to define them in an early stage.)}
\item Timing accurate model: more realistic. normal distribution, different shapes, with examples (sensor - normal, braking - only right side)

\item Name of I/O controller.
\end{itemize}


====== From 26th Aug,\\
\noindent (i) Motivation:
We are going to start our motivation from the uncertain computation times of I/Os. 
I have found some interesting paper published in Nature $<$Machine learning and computation-enabled intelligent sensor design$>$, which indicates that the modern sensors will be embedded with machine learning calculation -- this leads the I/O's computation time varies a lot. \textcolor{blue}{Great! This will give a very nice justification.}

\noindent (ii) Do we need to introduce the legends for each diagram? \textcolor{blue}{May be for Figure 3 only to save some space? \\
\textcolor{red}{It is not required.}\\}


======Paper Structure ====\\
{Sec. I. Intro, motivation, and related (1 page). \\}
{Sec. II. Hardware design (2 pages). \\}
{Sec. III. Scheduling/Optimisation (1 pages). \\}

System model - qualification of the timing accuracy. 

The timing accuracy of an I/O operation can be quantified by the absolute value of the difference between the time instant when the I/O operation is ideally expected to occur and the time instant when it actually occurs~\cite{jiang2017gpiocp,zhao2020timing}.

{Sec. IV \& V. Experimental Results, Conclusion, Reference (2.5 pages).}

\clearpage

==> intro_old.tex <==
\section{Introduction}
\label{sc:Introduction}
\zhenote{To do: revise the introduction and make the issue more critical and diffcult. \\}
\zhenote{I/O timing performance? \\}
Safety-critical systems have stringent assurance and verification requirements that are essential to emerging life-critical application scenarios, including medical, automotive, aerospace, and industrial automation~\cite{burns2001real}.
Input/Output (I/O) is a vital part of safety-critical systems~\cite{iso201126262,casini2021latency,hennessy2011computer}, in the sense that such systems rely on the I/Os to interface with sensors and actuators that need to either perceive a hazard in time or make manoeuvres to avoid a hazardous situation~\cite{borgioli2022virtualization}.
Therefore, it is necessary to guarantee that I/O operations behave \emph{correctly}, in a \emph{timing-predictable} manner --- meeting their deadline~\cite{casini2021latency}, and most importantly, with \emph{timing accuracy} --- getting executed at exact time instants (or at least within a small error margin)~\cite{zhao2020timing,jiang2017gpiocp}. 
Among these requirements, correctness and predictability have received much attention~\cite{casini2021latency,abdallah2016contention,missimer2016mixed,kim2014integrated,kim2018supporting}, however, timing accuracy has not been widely recognised~\cite{jiang2017gpiocp,zhao2020timing}.

The lack of timing accuracy often leads to imprecise control of I/O peripherals and less-effective data being collected from them~\cite{zhao2020timing,jiang2017gpiocp}.
In extreme cases, this can result in system failures and even cause catastrophic consequences~\cite{iso201126262}.
For instance, in spacecraft attitude control systems, the self-adaptive control algorithm requires a series of time-sensitive I/O operations to obtain and adjust the attitude of the spacecraft within a specific time margin~\cite{chai2019six}. 
Providing real-time guarantees for these I/O operations offers the foundation of the success of its mission, yet achieving precise I/O control (\ie, with timing accuracy) avoids accumulated deviations that can endanger the safety of the system, and is essential for accurate and stable attitude adjustments.
Therefore, I/O timing accuracy, as required by many industrial standards (\eg, DO-178C~\cite{rierson2017developing} and ISO 26262~\cite{iso201126262}), is crucial for system performance and safety.



Software approaches~\cite{abdallah2016contention,missimer2016mixed,kim2014integrated,betti2011real,kim2018supporting} typically integrate I/O-aware task scheduling and mapping strategies into Operating Systems (OSs) or hypervisors, minimising unnecessary I/O contentions. 
Through a comprehensive understanding of the system and in-depth analysis of I/O traffic, these approaches achieved a certain degree of timing guarantees. 
However, ensuring I/O timing accuracy has proven to be extremely difficult for these software approaches due to the ever-increasing hardware and architectural complexities, which introduce significant uncertainty to I/O transmissions, \eg, communication delays and resource contentions occurring from software applications (instigation) to hardware devices (execution)~\cite{jiang2017gpiocp}.
Hardware approaches~\cite{TPUWeb,PRUWeb,jiang2017gpiocp,zhao2020timing, casini2021latency, guerrra2008gravitational} usually employed dedicated assistance to manage I/O operations directly at the hardware level. 
By introducing restricted I/O scheduling close to the I/O devices, these approaches mitigated I/O transmission uncertainty, ensuring I/O timing accuracy under specific use-case scenarios.



\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{Overview.pdf}
    \vspace{-13pt}
    \caption{A conceptual overview of \name\ \emph{(square: router; circle: core; rectangle: \name; triangle: I/O device; curved arrows: I/O tasks with different timing guarantees)}: (a) \name\ serves as a co-processor, enabling I/O management at hardware; (b) \name\ features sets of ETSs and a two-level scheduler, limiting the impact of timing defects while offering a configurable scheduling infrastructure; (c) \nameS{} schedules tasks and configures \name\ using (d) customised commands, improving I/O robustness and accuracy.}
    \vspace{-10pt}
    \label{fig:concept}
\end{figure}

\parlabel{Research Challenge.}
However, to realise restricted I/O scheduling or management, these solutions rely on an idealistic assumption that ``\textit{the timing behaviours of the I/O operations must be well-defined}''~\cite{abdallah2016contention,missimer2016mixed,kim2014integrated,betti2011real,kim2018supporting,casini2021latency,jiang2017gpiocp, zhao2020timing}, including the Worst-Case Execution Time (WCET) and any interference to the I/O tasks.
In practice, \emph{unforeseen timing defects} can frequently occur for many reasons, \eg, 
ill-defined I/O-centric calculations~\cite{ballard2021machine} and unexpected transient failures caused by harsh environments~\cite{davis2007robust}.
With interference from timing defects, \eg, a task exceeding its WCET, the above approaches are fragile in which the complete task schedule would be entirely violated. 
Hence, these methods can guarantee neither accuracy nor predictability, which is challenging to achieve in real-world safety-critical systems with robustness taken into account. 
% In real-world safety-critical systems, it is important but challenging to achieve timing accuracy and robustness for real-time I/O control.

\parlabel{Contributions.}
This paper presents a systematical I/O management framework for robust and timing-accurate I/O control.
To achieve this, a novel I/O co-processor (\name{}) and a new scheduling method (\nameS) are constructed using a hardware/software co-designed approach, which guarantees predictability and improves accuracy in the presence of different timing defects. The contributions of this paper are summarised as follows:


\begin{itemize}
\item Configurable hardware-implemented Execution Time Servers (ETSs) in \name{} that provide temporal isolation for I/O tasks. 
This prohibits the propagation of timing defects.

\item A scalable two-level scheduler that manages I/O executions hierarchically using the ETSs. This establishes the scheduling infrastructure of \name{}.

\item An ETS-based scheduling method (\nameS{}) that dispatches I/O tasks and configures the ETSs to achieve real-time I/O control with timing accuracy and robustness.

\item A systematic I/O management framework, including both system architecture and programming methods, that
forms a complete solution based on \name{} and \nameS{}.
\end{itemize}

\noindent \textcolor{blue}{Experimental results show that, compared to the state-of-the-art real-time I/O controllers, \name{} improves both acceptance ratio and control quality by 22.61\% and 42.32\% on average (maximum: 2.18x and 3.06x), respectively. 
Synthesising a \name\ yields less than 10\% hardware overhead of a full-featured super-scalar processor.}
